Learning Fast Monomial Orders for Gr\"obner Basis Computations

The efficiency of Gr\"obner basis computation, the standard engine for solving systems of polynomial equations, depends on the choice of monomial ordering. Despite a near-continuum of possible monomial orders, most implementations rely on static heuristics such as GrevLex, guided primarily by expert intuition. We address this gap by casting the selection of monomial orderings as a reinforcement learning problem over the space of admissible orderings. Our approach leverages domain-informed reward signals that accurately reflect the computational cost of Gr\"obner basis computations and admits efficient Monte Carlo estimation. Experiments on benchmark problems from systems biology and computer vision show that the resulting learned policies consistently outperform standard heuristics, yielding substantial reductions in computational cost. Moreover, we find that these policies resist distillation into simple interpretable models, providing empirical evidence that deep reinforcement learning allows the agents to exploit non-linear geometric structure beyond the scope of traditional heuristics.

==> Grobner_and_F4.tex <==
In this section, we briefly review key mathematical concepts and notation; for further details see \cite{CoxLittleOShea2015}.

Let \(k\) be a field and \(R = k[x_1,\dots,x_n]\) the polynomial ring over \(k\). Fix a monomial ordering \(\prec\) on \(R\). For a nonzero polynomial \(f \in R\), denote by \(\mathrm{LM}_\prec(f)\) and \(\mathrm{LT}_\prec(f)\) its leading monomial and leading term, respectively.

\begin{definition}
A finite set \(G = \{g_1,\dots,g_t\} \subset I \subset R\) is a \emph{Gr\"obner basis} of \(I\) with respect to \(\prec\) if
\[
\langle \mathrm{LT}_\prec(g_1), \dots, \mathrm{LT}_\prec(g_t) \rangle
=
\langle \mathrm{LT}_\prec(I) \rangle.
\]
\end{definition}

A Gr\"obner basis is \emph{reduced} if each \(g_i\) is monic and no monomial of \(g_i\) is divisible by \(\mathrm{LM}_\prec(g_j)\) for \(j \neq i\). For a fixed monomial order, every ideal admits a unique reduced Gr\"obner basis \cite{CoxLittleOShea2015}. This does not imply, however, that every order will create a different reduced Gr\"obner basis as there are complex equivalences encoded by the Gr\"obner fan.

\subsection{Monomial Orderings and Weight Vectors}

A monomial ordering is a well-ordering on monomials that is compatible with multiplication. This means for every collection of monomials there will be a smallest one, and for any two monomials $x^{\alpha} =x_1^{\alpha_1} x_2^{\alpha_2} \cdots x_n^{\alpha_n}$ and $x^{\beta}=x_1^{\beta_1} \cdots x_n^{\beta_n}$ if $x^{\alpha}$ is ordered greater than $x^{\beta}$ then $x^{\alpha} x^{\gamma}= x^{\alpha+\gamma}$ should be ordered greater than $x^{\beta} x^{\gamma} = x^{\beta + \gamma}$. These properties ensure we can perform division and elimination properly, and guarantee
the termination of Gr\"obner basis algorithms.   

There is a convenient way to introduce monomial orders: Weight vectors \(w=(w_1,\dots,w_n)\in\mathbb{R}_{>0}^n\) can be used to create orderings via
\[
\deg_w(x^\alpha)=\sum_{i=1}^n w_i\alpha_i,
\]
with ties broken by a secondary order. Allowing real weights is natural when studying Gr\"obner fans, since this ordering is invariant under multiplying all coordinates of the weight vector with a fixed scalar. 

We mentioned that most current implementations only allow a few fixed monomial orders derived from expert intuition. These orderings are 
\begin{itemize}
    \item \textbf{Lex}: Lexicographic ordering starting from $x_1$ to $x_n$ (a limit of \(w=(M^{n-1},\dots,1)\), \(M\gg1\)),
    \item \textbf{GrLex}: This orders first with total degree and then breaks ties with lexicographic ordering (corresponding to \(w=(1,\dots,1)\)).
    \item \textbf{GrevLex}: This orders first with total degree and then breaks ties with reverse-lexicographic ordering (corresponding to \(w=(1,\dots,1)\)).
\end{itemize}
The choice of ordering strongly affects both the structure and the computational cost of the resulting Gr\"obner basis. There are theoretical and empirical results suggesting GrevLex is efficient, however, no general method exists for selecting an optimal order \cite{CoxLittleOShea2015}: this is precisely the blind spot in conventional wisdom that this paper aims to clarify.

\subsection{Buchberger's Algorithm and S-Polynomials}

Buchberger’s algorithm \cite{Buchberger2006} is based on \emph{S-polynomials}.

\begin{definition}
For nonzero \(f,g\in R\),
\[
S(f,g)=
\frac{\mathrm{lcm}(\mathrm{LM}(f),\mathrm{LM}(g))}{\mathrm{LT}(f)}f
-
\frac{\mathrm{lcm}(\mathrm{LM}(f),\mathrm{LM}(g))}{\mathrm{LT}(g)}g.
\]
\end{definition}

A generating set \(G\) is a Gr\"obner basis if and only if all S-polynomials reduce to zero modulo \(G\). Although conceptually simple, Buchberger’s algorithm can exhibit severe intermediate expression growth and doubly exponential worst-case complexity \cite{mayr1982complexity}. For graded reverse lexicographic orderings, sharper single-exponential degree bounds are known \cite{lazard1983,dube1990}, motivating their widespread use.

\subsection{The Gr\"obner Fan}

For a fixed ideal \(I \subset k[x_1,\dots,x_n]\), different monomial orders may yield distinct reduced Gr\"obner bases and initial ideals. The \emph{Gr\"obner fan} \cite{MoraRobbiano1988GrobnerFan,FukJensenThomas2007} provides a geometric framework for organizing this dependence using weight vectors \(w \in \mathbb{R}^n\). For \(f=\sum_\alpha c_\alpha x^\alpha\), the \(w\)-initial form \(\mathrm{in}_w(f)\) consists of terms with maximal \(\langle w,\alpha\rangle\), and the associated initial ideal is
\[
\mathrm{in}_w(I)=\langle \mathrm{in}_w(f): f\in I\rangle.
\]

As \(w\) varies, \(\mathrm{in}_w(I)\) remains constant on relatively open polyhedral cones and changes only when ties occur. These cones form a polyhedral fan whose full-dimensional cones are in bijection with the reduced Gr\"obner bases of \(I\). Classical orders such as Lex, GrLex, and GrevLex correspond to specific directions or refinements within this fan.

Figure~\ref{fig:grobner-fan-example} illustrates this structure schematically on a two-dimensional slice; it conveys how regions of constant initial ideal arise and how crossing a cone boundary corresponds to a combinatorial change in leading terms.

\medskip
\noindent\textbf{Example.}
Following Example~2.7 of \cite{FukJensenThomas2007}, consider
\[
I=\langle x+y+z,\; x^3z+x+y^2\rangle \subset \mathbb{Q}[x,y,z].
\]
With lexicographic order \(x\prec y\prec z\), a reduced Gr\"obner basis is
\[
G_{\mathrm{lex}}(I)=\{z+y+x,\; y^2+x-x^3y-x^4\},
\]
so \(\mathrm{in}_{\mathrm{lex}}(I)=\langle z,y^2\rangle\). The corresponding Gr\"obner cone consists of weight vectors satisfying linear inequalities ensuring that these leading terms persist; when one of these inequalities becomes tight, the initial ideal changes.

\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=5, line cap=round, line join=round]
  \coordinate (X) at (0,0);
  \coordinate (Y) at (1,0);
  \coordinate (Z) at (0.5,0.8660254);

  \coordinate (C)  at (0.5,0.2886751);
  \coordinate (P)  at (0.7142857,0.3711537);

  % Outer simplex
  \draw[thick] (X)--(Y)--(Z)--cycle;
  \fill[gray!10] (X)--(Y)--(Z)--cycle;

  % Vertex labels
  \node[below left]  at (X) {$w_1$};
  \node[below right] at (Y) {$w_2$};
  \node[above]       at (Z) {$w_3$};

  % Internal rays (slightly shortened)
  \draw[thick] (C) -- ($(X)!0.48!(Z)$);
  \draw[thick] (C) -- ($(Y)!0.48!(Z)$);
  \draw[thick] (C) -- ($(X)!0.48!(Y)$);

  % Center point
  \fill (C) circle(0.0045);
  \node[xshift=-1spt,yshift=11pt] at (C)
    {\scriptsize $(\tfrac13,\tfrac13,\tfrac13)$};

  % Interior point
  \fill (P) circle(0.0045);
  \node[xshift=4pt,yshift=-9pt] at (P)
    {\scriptsize $(\tfrac17,\tfrac37,\tfrac37)$};

  % Initial ideal label (moved to open region)
  \node at (0.28,0.12)
    {\scriptsize $\mathrm{in}_w(I)=\langle z,y^2\rangle$};
\end{tikzpicture}
\caption{A schematic two-dimensional slice ($w_1+w_2+w_3=1$, $w\ge0$) of the Gr\"obner fan for
\(I=\langle x+y+z,\;x^3z+x+y^2\rangle\), illustrating how regions of constant
\(\mathrm{in}_w(I)\) arise. The diagram is not to scale and is intended to convey
the geometric structure of cones rather than exact fan boundaries; see
\cite{FukJensenThomas2007}.}
\label{fig:grobner-fan-example}
\end{figure}


\subsection{The FGLM and \(F_4\) Algorithms}

For zero-dimensional ideals \(I\), where \(R/I\) is finite-dimensional, the FGLM algorithm \cite{FGLM1993} converts a Gr\"obner basis under a degree-compatible order into one under another order using linear algebra. Modern variants are commonly used to transform from a fast monomial ordering to Lex, and the computation is effective in applications; see \cite{FaugereMou2017SparseFGLM,berthomieu2022faster}.

Faug\`ere’s \(F_4\) algorithm \cite{Faugere1999F4} accelerates Buchberger’s method by batching reductions and performing them via structured linear algebra. At each stage, selected S-polynomials and multiples of basis elements are assembled into a matrix whose rows correspond to polynomials and columns to monomials. A subroutine of \(F_4\) called symbolic preprocessing constructs this matrix, after which reduction is performed by Gaussian elimination. \(F_4\) exploits the specific sparsity patterns of these matrices for high performance. 

The dominant cost of \(F_4\) is governed by the dimensions of these matrices. In particular, the number of columns, denoted by \(n_M\) in our reward formulation, captures the size of the active monomial basis and directly determines memory usage and linear algebra cost. Degree growth increases these dimensions and depends strongly on the monomial order. Since computation proceeds incrementally through such matrix constructions, these quantities provide natural proxies for computational effort and are used as feedback signals in our RL environment design.

